Global property prediction: A benchmark study on open source, perovskite-like datasets

Screening combinatorial space for novel materials - such as perovskite-like ones for photovoltaics - has resulted in a high amount of simulated high-troughput data and analysis thereof. This study proposes a comprehensive comparison of structural-fingerprint based machine-learning models on seven open-source databases of perovskite-like materials to predict bandgaps and energies. It shows that none of the given methods are able to capture arbitrary databases evenly, while underlining that commonly used metrics are highly database dependent in typical workflows. In addition the applicability of variance selection and autoencoders to significantly reduce fingerprint size indicates that models built with common fingerprints only rely on a submanifold of the available fingerprint space.

==> energy_maes.tex <==
\begin{tabular}{lccc}
\toprule
{} & Kim \cite{Kim2017} & Sutton \cite{Sutton2019} & Stan. \cite{Stanley2019} \\
\midrule
handpicked                 &          109.1±5.9 &                        - &                        - \\
dummy                      &         262.0±10.1 &                 34.3±1.0 &               119.1±11.7 \\
sinematrix, eigenspectrum  &           70.7±3.7 &                 10.5±0.3 &                 38.8±7.4 \\
PDDF, basic                &            4.8±0.3 &                  6.3±0.3 &                  4.5±0.5 \\
PDDF, fine                 &            3.5±0.7 &                  4.4±0.3 &                  3.0±0.5 \\
PDDF, fine+AE              &            4.2±0.3 &                  4.6±0.3 &                  3.8±0.3 \\
P²DDF, basic               &            3.9±0.3 &                  5.9±0.3 &                  5.6±0.7 \\
P²DDF, fine                &            2.7±0.3 &                  3.7±0.2 &                  3.6±0.9 \\
P²DDF, fine+AE             &            3.8±0.5 &                  4.3±0.3 &                  4.4±0.8 \\
MBTR, k2-inv               &            2.1±0.3 &                  2.0±0.1 &                  2.7±0.3 \\
MBTR, k2-rdf               &            2.6±0.3 &                  2.5±0.1 &                  2.7±0.2 \\
MBTR, k2-inv-100           &            2.0±0.3 &                  1.9±0.2 &                  2.6±0.2 \\
MBTR, k2-rdf-100           &            2.8±0.3 &                  2.2±0.1 &                  2.6±0.2 \\
MBTR, k2-inv-broad         &            3.0±0.3 &                  5.4±0.4 &                  3.6±0.4 \\
MBTR, k2-rdf-broad         &            3.9±1.0 &                  6.1±0.3 &                  3.1±0.4 \\
MBTR, full                 &            2.0±0.2 &                  1.9±0.1 &                  2.7±0.3 \\
MBTR, k2-inv+varsel        &            2.4±0.2 &                  2.0±0.1 &                  3.1±0.6 \\
MBTR, k2-rdf+varsel        &            5.0±0.3 &                  2.8±0.1 &                  4.0±0.5 \\
MBTR, k2-inv-broad+varsel  &            4.8±0.8 &                  5.8±0.3 &                  3.4±0.3 \\
MBTR, k2-rdf-broad+varsel  &            5.6±0.5 &                  5.3±0.2 &                  3.1±0.4 \\
MBTR, k2-inv-100+varsel    &            2.6±0.2 &                  2.0±0.1 &                  4.0±0.6 \\
MBTR, k2-rdf-100+varsel    &            5.7±0.4 &                  3.0±0.1 &                  4.5±0.7 \\
MBTR, full+varsel          &            4.0±0.3 &                  2.0±0.1 &                 10.3±7.9 \\
SOAP, Marchenko            &            6.9±0.6 &                  0.7±0.1 &                  4.0±0.4 \\
SOAP, De                   &            5.3±0.7 &                  0.7±0.1 &                  2.5±0.4 \\
SOAP, Nomad                &            3.8±0.4 &                  0.7±0.0 &                  2.6±0.2 \\
SOAP, Nomad, fine          &            8.5±0.4 &                 12.8±0.2 &                  3.7±0.6 \\
SOAP, Marchenko, LR        &           10.1±1.1 &                  1.4±0.1 &                  7.0±0.7 \\
SOAP, Marchenko+varsel     &            3.4±0.4 &                  1.4±0.1 &                  7.0±0.6 \\
SOAP, De+varsel            &            4.9±0.5 &                  1.6±0.1 &                  4.5±0.5 \\
SOAP, Nomad+varsel         &            2.5±0.2 &                  1.1±0.1 &                  4.6±0.6 \\
SOAP, Nomad, fine+varsel   &            2.5±0.2 &                  1.2±0.1 &                  4.4±0.5 \\
SOAP, Marchenko, LR+varsel &            4.5±0.4 &                  1.5±0.1 &                  7.7±0.9 \\
\bottomrule
\end{tabular}


==> energy_r2s.tex <==
\begin{tabular}{lccc}
\toprule
{} &                                 Kim \cite{Kim2017} &                           Sutton \cite{Sutton2019} &                           Stan. \cite{Stanley2019} \\
\midrule
handpicked                 &                                          0.72±0.05 &                                                  - &                                                  - \\
dummy                      &   - & - & -  \\
sinematrix, eigenspectrum  &                                          0.90±0.01 &                                          0.80±0.04 &                                          0.73±0.17 \\
PDDF, basic                &                                          1.00±0.00 &                                          0.93±0.01 &                                          1.00±0.00 \\
PDDF, fine                 &                                          1.00±0.00 &                                          0.97±0.01 &                                          1.00±0.00 \\
PDDF, fine+AE              &                                          1.00±0.00 &                                          0.96±0.01 &                                          1.00±0.00 \\
P²DDF, basic               &                                          1.00±0.00 &                                          0.94±0.01 &                                          1.00±0.00 \\
P²DDF, fine                &                                          1.00±0.00 &                                          0.97±0.01 &                                          1.00±0.00 \\
P²DDF, fine+AE             &                                          1.00±0.00 &                                          0.97±0.01 &                                          1.00±0.00 \\
MBTR, k2-inv               &                                          1.00±0.00 &                                          0.99±0.01 &                                          1.00±0.00 \\
MBTR, k2-rdf               &                                          1.00±0.00 &                                          0.99±0.01 &                                          1.00±0.00 \\
MBTR, k2-inv-100           &                                          1.00±0.00 &                                          0.99±0.01 &                                          1.00±0.00 \\
MBTR, k2-rdf-100           &                                          1.00±0.00 &                                          0.99±0.00 &                                          1.00±0.00 \\
MBTR, k2-inv-broad         &                                          1.00±0.00 &                                          0.95±0.03 &                                          1.00±0.00 \\
MBTR, k2-rdf-broad         &                                          1.00±0.00 &                                          0.94±0.03 &                                          1.00±0.00 \\
MBTR, full                 &                                          1.00±0.00 &                                          0.99±0.01 &                                          1.00±0.00 \\
MBTR, k2-inv+varsel        &                                          1.00±0.00 &                                          0.99±0.00 &                                          1.00±0.00 \\
MBTR, k2-rdf+varsel        &                                          1.00±0.00 &                                          0.99±0.00 &                                          1.00±0.00 \\
MBTR, k2-inv-broad+varsel  &                                          1.00±0.00 &                                          0.95±0.02 &                                          1.00±0.00 \\
MBTR, k2-rdf-broad+varsel  &                                          1.00±0.00 &                                          0.96±0.01 &                                          1.00±0.00 \\
MBTR, k2-inv-100+varsel    &                                          1.00±0.00 &                                          0.99±0.00 &                                          1.00±0.00 \\
MBTR, k2-rdf-100+varsel    &                                          1.00±0.00 &                                          0.99±0.00 &                                          1.00±0.00 \\
MBTR, full+varsel          &                                          1.00±0.00 &                                          0.99±0.00 &                                          0.93±0.13 \\
SOAP, Marchenko            &                                          1.00±0.00 &                                          1.00±0.00 &                                          1.00±0.00 \\
SOAP, De                   &                                          1.00±0.00 &                                          1.00±0.00 &                                          1.00±0.00 \\
SOAP, Nomad                &                                          1.00±0.00 &                                          1.00±0.00 &                                          1.00±0.00 \\
SOAP, Nomad, fine          &                                          1.00±0.00 &                                          0.75±0.02 &                                          1.00±0.00 \\
SOAP, Marchenko, LR        &                                          1.00±0.00 &                                          0.99±0.00 &                                          1.00±0.00 \\
SOAP, Marchenko+varsel     &                                          1.00±0.00 &                                          1.00±0.00 &                                          1.00±0.00 \\
SOAP, De+varsel            &                                          1.00±0.00 &                                          0.99±0.00 &                                          1.00±0.00 \\
SOAP, Nomad+varsel         &                                          1.00±0.00 &                                          1.00±0.00 &                                          1.00±0.00 \\
SOAP, Nomad, fine+varsel   &                                          1.00±0.00 &                                          1.00±0.00 &                                          1.00±0.00 \\
SOAP, Marchenko, LR+varsel &                                          1.00±0.00 &                                          1.00±0.00 &                                          0.99±0.00 \\
\bottomrule
\end{tabular}


==> energy_rmses.tex <==
\begin{tabular}{lccc}
\toprule
{} & Kim \cite{Kim2017} & Sutton \cite{Sutton2019} & Stan. \cite{Stanley2019} \\
\midrule
handpicked                 &         160.3±10.1 &                        - &                        - \\
dummy                      &         346.7±11.3 &                 41.9±1.2 &               147.5±13.5 \\
sinematrix, eigenspectrum  &          103.6±7.2 &                 17.2±1.3 &                84.1±42.0 \\
PDDF, basic                &            7.6±1.0 &                 10.6±1.0 &                  5.9±0.7 \\
PDDF, fine                 &            5.5±0.9 &                  7.6±0.7 &                  4.1±1.0 \\
PDDF, fine+AE              &            6.2±0.5 &                  7.8±0.7 &                  5.1±0.7 \\
P²DDF, basic               &            5.7±0.5 &                  9.9±1.2 &                  7.7±1.1 \\
P²DDF, fine                &            3.9±0.6 &                  6.5±1.0 &                  5.1±1.6 \\
P²DDF, fine+AE             &            5.7±1.0 &                  7.4±0.8 &                  5.9±1.3 \\
MBTR, k2-inv               &            3.2±0.3 &                  3.9±1.3 &                  4.6±0.9 \\
MBTR, k2-rdf               &            4.0±0.5 &                  4.6±0.9 &                  4.3±1.0 \\
MBTR, k2-inv-100           &            3.2±0.4 &                  3.6±1.1 &                  4.5±1.0 \\
MBTR, k2-rdf-100           &            4.1±0.5 &                  4.0±0.4 &                  4.3±1.0 \\
MBTR, k2-inv-broad         &            4.5±0.4 &                  8.7±2.0 &                  5.1±1.1 \\
MBTR, k2-rdf-broad         &            5.9±1.4 &                  9.6±2.2 &                  4.5±0.9 \\
MBTR, full                 &            3.1±0.2 &                  3.7±1.2 &                  4.6±0.9 \\
MBTR, k2-inv+varsel        &            4.2±0.5 &                  3.6±0.8 &                  4.7±1.5 \\
MBTR, k2-rdf+varsel        &            7.7±0.8 &                  4.6±0.6 &                  5.8±1.1 \\
MBTR, k2-inv-broad+varsel  &            6.9±1.0 &                  9.1±1.4 &                  4.8±0.7 \\
MBTR, k2-rdf-broad+varsel  &            8.7±2.3 &                  8.4±0.9 &                  4.5±1.0 \\
MBTR, k2-inv-100+varsel    &            4.3±0.6 &                  3.6±0.5 &                  6.0±1.9 \\
MBTR, k2-rdf-100+varsel    &            8.4±0.6 &                  4.9±0.6 &                  6.4±1.6 \\
MBTR, full+varsel          &            6.2±0.8 &                  3.3±0.3 &                29.3±42.7 \\
SOAP, Marchenko            &           12.5±1.7 &                  1.5±0.4 &                  5.3±0.6 \\
SOAP, De                   &            9.9±1.3 &                  1.3±0.5 &                  3.5±0.9 \\
SOAP, Nomad                &            7.1±1.0 &                  1.4±0.5 &                  3.5±0.5 \\
SOAP, Nomad, fine          &           12.6±0.8 &                 17.0±0.4 &                  5.1±1.2 \\
SOAP, Marchenko, LR        &           19.9±3.0 &                  3.2±0.4 &                  9.9±1.6 \\
SOAP, Marchenko+varsel     &            5.7±0.7 &                  2.7±0.7 &                  9.6±1.8 \\
SOAP, De+varsel            &            7.8±1.1 &                  3.3±0.7 &                  6.2±0.9 \\
SOAP, Nomad+varsel         &            4.1±0.4 &                  2.4±0.8 &                  6.3±1.0 \\
SOAP, Nomad, fine+varsel   &            4.1±0.5 &                  2.2±0.4 &                  5.9±0.6 \\
SOAP, Marchenko, LR+varsel &            7.1±0.7 &                  2.9±0.7 &                 11.0±2.0 \\
\bottomrule
\end{tabular}


==> gap_maes.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & Kim \cite{Kim2017} & Pandey \cite{Pandey2018} & Stan. \cite{Stanley2019} & Cas. \cite{Castelli2012_cubic} & Cas. \cite{Castelli2013_lowsymm} & Mar. \cite{Marchenko2020} & Sutton \cite{Sutton2019} \\
\midrule
handpicked                 &             381±11 &                        - &                        - &                              - &                                - &                         - &                        - \\
dummy                      &             884±34 &                   730±19 &                   323±23 &                        1270±73 &                          1530±46 &                    332±15 &                   845±16 \\
sinematrix, eigenspectrum  &             368±15 &                   538±39 &                   212±15 &                        1088±77 &                          1102±60 &                    298±22 &                    141±8 \\
PDDF, basic                &             172±11 &                   199±13 &                   134±11 &                         930±80 &                           551±16 &                    179±11 &                    101±4 \\
PDDF, fine                 &              141±8 &                   139±14 &                   114±12 &                         888±57 &                           481±19 &                    176±20 &                     90±4 \\
PDDF, fine+AE              &              142±6 &                    143±7 &                   110±12 &                         879±61 &                           490±28 &                    170±19 &                     91±4 \\
P²DDF, basic               &             159±12 &                   172±14 &                   136±19 &                         888±69 &                           521±19 &                    207±32 &                     96±3 \\
P²DDF, fine                &             118±12 &                    116±9 &                    109±7 &                         834±55 &                           436±22 &                    176±29 &                     85±3 \\
P²DDF, fine+AE             &              120±7 &                    113±8 &                    109±6 &                         806±48 &                           421±27 &                    178±31 &                     91±2 \\
MBTR, k2-inv               &              124±7 &                   159±12 &                   120±11 &                         709±50 &                           260±15 &                    143±11 &                     90±5 \\
MBTR, k2-rdf               &              128±7 &                   144±13 &                   126±10 &                         786±57 &                           305±18 &                    140±18 &                     93±6 \\
MBTR, k2-inv-100           &              124±6 &                   160±13 &                   120±11 &                         705±52 &                           262±16 &                    145±11 &                     89±5 \\
MBTR, k2-rdf-100           &              127±8 &                   146±14 &                   125±10 &                         787±59 &                           301±17 &                    146±14 &                     95±6 \\
MBTR, k2-inv-broad         &             171±11 &                    283±8 &                   131±13 &                         867±62 &                           362±19 &                    149±15 &                    125±7 \\
MBTR, k2-rdf-broad         &             159±10 &                   228±23 &                   133±12 &                         875±60 &                           345±18 &                    148±13 &                    112±7 \\
MBTR, full                 &              124±7 &                   158±13 &                   120±11 &                         709±52 &                           260±16 &                    141±12 &                     89±5 \\
MBTR, k2-inv+varsel        &              125±8 &                   178±12 &                   126±14 &                         768±63 &                           348±27 &                    142±15 &                     86±4 \\
MBTR, k2-rdf+varsel        &             149±10 &                    164±9 &                   154±13 &                         835±67 &                           394±22 &                    139±13 &                     95±5 \\
MBTR, k2-inv-broad+varsel  &             178±12 &                   286±12 &                   133±11 &                         967±81 &                           435±25 &                    132±22 &                   127±11 \\
MBTR, k2-rdf-broad+varsel  &             156±10 &                   255±18 &                   138±14 &                         926±39 &                           422±37 &                    127±19 &                   116±10 \\
MBTR, k2-inv-100+varsel    &              125±7 &                   177±12 &                   124±15 &                         766±59 &                           350±26 &                    151±18 &                     88±5 \\
MBTR, k2-rdf-100+varsel    &              154±9 &                    168±9 &                    153±9 &                         822±49 &                           392±25 &                    151±26 &                     99±5 \\
MBTR, full+varsel          &              112±8 &                    130±8 &                   140±21 &                         771±44 &                           331±25 &                    148±22 &                     89±6 \\
SOAP, Marchenko            &              100±8 &                     85±9 &                    109±7 &                        1067±75 &                           349±27 &                    494±90 &                     70±5 \\
SOAP, De                   &              107±6 &                     97±9 &                    108±8 &                        1071±74 &                           329±25 &                    442±95 &                     78±4 \\
SOAP, Nomad                &              106±7 &                     90±8 &                   104±10 &                         926±64 &                           352±27 &                   339±112 &                     72±4 \\
SOAP, Nomad, fine          &             195±11 &                    281±8 &                   181±13 &                         823±68 &                           443±23 &                    144±17 &                    149±8 \\
SOAP, Marchenko, LR        &             110±11 &                     96±7 &                   122±10 &                       1288±130 &                           645±58 &                   939±330 &                     75±3 \\
SOAP, Marchenko+varsel     &              101±6 &                   111±10 &                    123±8 &                         738±52 &                           309±24 &                    132±17 &                     77±6 \\
SOAP, De+varsel            &              106±9 &                   112±10 &                    116±7 &                         777±50 &                           339±23 &                    135±20 &                     78±4 \\
SOAP, Nomad+varsel         &              105±6 &                   114±11 &                    110±9 &                         734±45 &                           327±18 &                    125±18 &                     76±2 \\
SOAP, Nomad, fine+varsel   &              106±6 &                   117±10 &                    110±8 &                         731±48 &                           316±17 &                    146±36 &                     77±4 \\
SOAP, Marchenko, LR+varsel &               99±8 &                     90±5 &                    104±8 &                         745±48 &                           324±27 &                    129±25 &                     76±3 \\
\bottomrule
\end{tabular}


==> gap_maes_main_old.tex <==
\begin{tabular}{rccccccc}
\toprule
{} & Kim \cite{Kim2017} & Pandey \cite{Pandey2018} & Stan. \cite{Stanley2019} & Cas. \cite{Castelli2012_cubic} & Cas. \cite{Castelli2013_lowsymm} & Mar. \cite{Marchenko2020} & Sutton \cite{Sutton2019} \\
\midrule
dummy                      &             884±34 &                   730±19 &                   323±23 &                        1270±73 &                          1530±46 &                    332±15 &                   845±16 \\
sinematrix, eigenspectrum  &             368±15 &                   538±39 &                   212±15 &                        1088±77 &                          1102±60 &                    298±22 &                    141±8 \\
PDDF, basic                &             172±11 &                   199±13 &                   134±11 &                         930±80 &                           551±16 &                    179±11 &                    101±4 \\
PDDF, fine                 &              141±8 &                   139±14 &                   114±12 &                         888±57 &                           481±19 &                    176±20 &                     90±4 \\
PDDF, fine+AE              &              142±6 &                    143±7 &                   110±12 &                         879±61 &                           490±28 &                    170±19 &                     91±4 \\
P²DDF, basic               &             159±12 &                   172±14 &                   136±19 &                         888±69 &                           521±19 &                    207±32 &                     96±3 \\
P²DDF, fine                &             118±12 &                    116±9 &                    109±7 &                         834±55 &                           436±22 &                    176±29 &                     85±3 \\
P²DDF, fine+AE             &              120±7 &                    113±8 &                    109±6 &                         806±48 &                           421±27 &                    178±31 &                     91±2 \\
MBTR, k2-inv               &              124±7 &                   159±12 &                   120±11 &                         709±50 &                           260±15 &                    143±11 &                     90±5 \\
MBTR, k2-rdf               &              128±7 &                   144±13 &                   126±10 &                         786±57 &                           305±18 &                    140±18 &                     93±6 \\
MBTR, k2-inv-broad         &             171±11 &                    283±8 &                   131±13 &                         867±62 &                           362±19 &                    149±15 &                    125±7 \\
MBTR, k2-rdf-broad         &             159±10 &                   228±23 &                   133±12 &                         875±60 &                           345±18 &                    148±13 &                    112±7 \\
MBTR, k2-inv+varsel        &              125±8 &                   178±12 &                   126±14 &                         768±63 &                           348±27 &                    142±15 &                     86±4 \\
MBTR, k2-rdf+varsel        &             149±10 &                    164±9 &                   154±13 &                         835±67 &                           394±22 &                    139±13 &                     95±5 \\
MBTR, k2-inv-broad+varsel  &             178±12 &                   286±12 &                   133±11 &                         967±81 &                           435±25 &                    132±22 &                   127±11 \\
MBTR, k2-rdf-broad+varsel  &             156±10 &                   255±18 &                   138±14 &                         926±39 &                           422±37 &                    127±19 &                   116±10 \\
MBTR, k2-inv-100+varsel    &              125±7 &                   177±12 &                   124±15 &                         766±59 &                           350±26 &                    151±18 &                     88±5 \\
MBTR, k2-rdf-100+varsel    &              154±9 &                    168±9 &                    153±9 &                         822±49 &                           392±25 &                    151±26 &                     99±5 \\
MBTR, full+varsel          &              112±8 &                    130±8 &                   140±21 &                         771±44 &                           331±25 &                    148±22 &                     89±6 \\
SOAP, Marchenko+varsel     &              101±6 &                   111±10 &                    123±8 &                         738±52 &                           309±24 &                    132±17 &                     77±6 \\
SOAP, De+varsel            &              106±9 &                   112±10 &                    116±7 &                         777±50 &                           339±23 &                    135±20 &                     78±4 \\
SOAP, Nomad+varsel         &              105±6 &                   114±11 &                    110±9 &                         734±45 &                           327±18 &                    125±18 &                     76±2 \\
SOAP, Nomad, fine+varsel   &              106±6 &                   117±10 &                    110±8 &                         731±48 &                           316±17 &                    146±36 &                     77±4 \\
SOAP, Marchenko, LR+varsel &               99±8 &                     90±5 &                    104±8 &                         745±48 &                           324±27 &                    129±25 &                     76±3 \\
SOAP, Marchenko            &              100±8 &                     85±9 &                    109±7 &                        1067±75 &                           349±27 &                    494±90 &                     70±5 \\
SOAP, De                   &              107±6 &                     97±9 &                    108±8 &                        1071±74 &                           329±25 &                    442±95 &                     78±4 \\
SOAP, Nomad                &              106±7 &                     90±8 &                   104±10 &                         926±64 &                           352±27 &                   339±112 &                     72±4 \\
SOAP, Nomad, fine          &             195±11 &                    281±8 &                   181±13 &                         823±68 &                           443±23 &                    144±17 &                    149±8 \\
SOAP, Marchenko, LR        &             110±11 &                     96±7 &                   122±10 &                       1288±130 &                           645±58 &                   939±330 &                     75±3 \\
MBTR, k2-inv-100           &              124±6 &                   160±13 &                   120±11 &                         705±52 &                           262±16 &                    145±11 &                     89±5 \\
MBTR, k2-rdf-100           &              127±8 &                   146±14 &                   125±10 &                         787±59 &                           301±17 &                    146±14 &                     95±6 \\
MBTR, full                 &              124±7 &                   158±13 &                   120±11 &                         709±52 &                           260±16 &                    141±12 &                     89±5 \\
\bottomrule
\end{tabular}


==> gap_r2s.tex <==
\begin{tabular}{lccccccc}
\toprule
{} &                                 Kim \cite{Kim2017} &                           Pandey \cite{Pandey2018} &                           Stan. \cite{Stanley2019} &                     Cas. \cite{Castelli2012_cubic} &                   Cas. \cite{Castelli2013_lowsymm} &                          Mar. \cite{Marchenko2020} &                           Sutton \cite{Sutton2019} \\
\midrule
handpicked                 &                                          0.79±0.01 &                                                  - &                                                  - &                                                  - &                                                  - &                                                  - &                                                  - \\
dummy                      &  - &                                                  - &                                                  - &                                                  - &                                                  - &                                                  - &                                                  - \\
sinematrix, eigenspectrum  &                                          0.75±0.03 &                                         -0.01±0.33 &                                          0.09±0.18 &                                         -2.21±0.73 &                                          0.04±0.15 &                                         -3.78±2.06 &                                          0.95±0.01 \\
PDDF, basic                &                                          0.95±0.01 &                                          0.89±0.02 &                                          0.72±0.08 &                                         -0.06±0.25 &                                          0.80±0.02 &                                          0.55±0.10 &                                          0.97±0.00 \\
PDDF, fine                 &                                          0.97±0.00 &                                          0.94±0.01 &                                          0.82±0.05 &                                          0.15±0.16 &                                          0.84±0.02 &                                          0.53±0.13 &                                          0.98±0.01 \\
PDDF, fine+AE              &                                          0.97±0.00 &                                          0.94±0.01 &                                          0.83±0.06 &                                          0.17±0.15 &                                          0.83±0.02 &                                          0.58±0.14 &                                          0.98±0.00 \\
P²DDF, basic               &                                          0.96±0.01 &                                          0.92±0.02 &                                          0.69±0.12 &                                          0.06±0.20 &                                          0.80±0.03 &                                          0.35±0.22 &                                          0.98±0.00 \\
P²DDF, fine                &                                          0.97±0.01 &                                          0.96±0.01 &                                          0.86±0.03 &                                          0.24±0.13 &                                          0.86±0.02 &                                          0.49±0.21 &                                          0.98±0.00 \\
P²DDF, fine+AE             &                                          0.97±0.00 &                                          0.96±0.01 &                                          0.85±0.03 &                                          0.36±0.07 &                                          0.87±0.02 &                                          0.50±0.21 &                                          0.98±0.00 \\
MBTR, k2-inv               &                                          0.97±0.00 &                                          0.92±0.02 &                                          0.83±0.05 &                                          0.50±0.09 &                                          0.94±0.01 &                                          0.67±0.11 &                                          0.98±0.00 \\
MBTR, k2-rdf               &                                          0.97±0.00 &                                          0.93±0.02 &                                          0.81±0.05 &                                          0.30±0.09 &                                          0.92±0.01 &                                          0.71±0.14 &                                          0.98±0.00 \\
MBTR, k2-inv-100           &                                          0.97±0.00 &                                          0.92±0.02 &                                          0.82±0.05 &                                          0.49±0.09 &                                          0.94±0.01 &                                          0.67±0.09 &                                          0.98±0.00 \\
MBTR, k2-rdf-100           &                                          0.97±0.00 &                                          0.93±0.02 &                                          0.81±0.06 &                                          0.30±0.10 &                                          0.92±0.01 &                                          0.65±0.14 &                                          0.98±0.00 \\
MBTR, k2-inv-broad         &                                          0.95±0.01 &                                          0.75±0.03 &                                          0.79±0.07 &                                         -0.05±0.13 &                                          0.90±0.02 &                                          0.64±0.15 &                                          0.96±0.01 \\
MBTR, k2-rdf-broad         &                                          0.96±0.01 &                                          0.84±0.03 &                                          0.77±0.07 &                                         -0.08±0.14 &                                          0.91±0.01 &                                          0.65±0.15 &                                          0.97±0.01 \\
MBTR, full                 &                                          0.97±0.00 &                                          0.92±0.02 &                                          0.83±0.05 &                                          0.50±0.09 &                                          0.94±0.01 &                                          0.67±0.12 &                                          0.98±0.00 \\
MBTR, k2-inv+varsel        &                                          0.97±0.00 &                                          0.91±0.02 &                                          0.79±0.06 &                                          0.40±0.11 &                                          0.89±0.02 &                                          0.65±0.13 &                                          0.98±0.00 \\
MBTR, k2-rdf+varsel        &                                          0.96±0.00 &                                          0.92±0.01 &                                          0.65±0.05 &                                          0.33±0.11 &                                          0.87±0.03 &                                          0.71±0.11 &                                          0.98±0.00 \\
MBTR, k2-inv-broad+varsel  &                                          0.95±0.01 &                                          0.74±0.04 &                                          0.79±0.05 &                                         -0.07±0.23 &                                          0.85±0.05 &                                          0.74±0.16 &                                          0.96±0.01 \\
MBTR, k2-rdf-broad+varsel  &                                          0.96±0.01 &                                          0.80±0.04 &                                          0.75±0.07 &                                          0.14±0.12 &                                          0.86±0.04 &                                          0.75±0.15 &                                          0.96±0.01 \\
MBTR, k2-inv-100+varsel    &                                          0.97±0.00 &                                          0.91±0.01 &                                          0.80±0.05 &                                          0.40±0.11 &                                          0.89±0.02 &                                          0.55±0.14 &                                          0.98±0.01 \\
MBTR, k2-rdf-100+varsel    &                                          0.96±0.00 &                                          0.91±0.01 &                                          0.66±0.06 &                                          0.36±0.12 &                                          0.87±0.03 &                                          0.63±0.19 &                                          0.98±0.00 \\
MBTR, full+varsel          &                                          0.97±0.01 &                                          0.93±0.02 &                                          0.67±0.23 &                                          0.47±0.11 &                                          0.90±0.02 &                                          0.59±0.15 &                                          0.98±0.00 \\
SOAP, Marchenko            &                                          0.98±0.00 &                                          0.97±0.01 &                                          0.86±0.02 &                                          0.29±0.11 &                                          0.86±0.03 &                                          0.11±0.14 &                                          0.99±0.00 \\
SOAP, De                   &                                          0.98±0.00 &                                          0.96±0.01 &                                          0.87±0.04 &                                          0.29±0.11 &                                          0.89±0.02 &                                          0.15±0.13 &                                          0.98±0.00 \\
SOAP, Nomad                &                                          0.98±0.00 &                                          0.96±0.01 &                                          0.87±0.03 &                                          0.33±0.12 &                                          0.91±0.01 &                                          0.23±0.23 &                                          0.99±0.00 \\
SOAP, Nomad, fine          &                                          0.94±0.01 &                                          0.76±0.03 &                                          0.38±0.12 &                                          0.25±0.19 &                                          0.87±0.02 &                                          0.70±0.09 &                                          0.94±0.01 \\
SOAP, Marchenko, LR        &                                          0.97±0.01 &                                          0.95±0.01 &                                          0.84±0.03 &                                          0.18±0.10 &                                          0.49±0.07 &                                          0.04±0.07 &                                          0.98±0.00 \\
SOAP, Marchenko+varsel     &                                          0.98±0.00 &                                          0.94±0.02 &                                          0.82±0.03 &                                          0.50±0.07 &                                          0.91±0.02 &                                          0.67±0.18 &                                          0.98±0.01 \\
SOAP, De+varsel            &                                          0.98±0.00 &                                          0.95±0.01 &                                          0.84±0.03 &                                          0.36±0.09 &                                          0.90±0.02 &                                          0.67±0.13 &                                          0.98±0.00 \\
SOAP, Nomad+varsel         &                                          0.98±0.00 &                                          0.95±0.02 &                                          0.85±0.02 &                                          0.43±0.11 &                                          0.91±0.02 &                                          0.68±0.16 &                                          0.98±0.00 \\
SOAP, Nomad, fine+varsel   &                                          0.98±0.00 &                                          0.94±0.02 &                                          0.86±0.03 &                                          0.47±0.10 &                                          0.91±0.01 &                                          0.58±0.28 &                                          0.98±0.00 \\
SOAP, Marchenko, LR+varsel &                                          0.98±0.00 &                                          0.96±0.01 &                                          0.86±0.03 &                                          0.48±0.06 &                                          0.90±0.03 &                                          0.67±0.18 &                                          0.98±0.00 \\
\bottomrule
\end{tabular}


==> gap_rmses.tex <==
\begin{tabular}{lccccccc}
\toprule
{} & Kim \cite{Kim2017} & Pandey \cite{Pandey2018} & Stan. \cite{Stanley2019} & Cas. \cite{Castelli2012_cubic} & Cas. \cite{Castelli2013_lowsymm} & Mar. \cite{Marchenko2020} & Sutton \cite{Sutton2019} \\
\midrule
handpicked                 &              446±8 &                        - &                        - &                              - &                                - &                         - &                        - \\
dummy                      &            1073±40 &                   887±19 &                   429±32 &                       1580±114 &                          1870±48 &                    414±23 &                  1020±26 \\
sinematrix, eigenspectrum  &             485±19 &                   681±50 &                   293±24 &                        1396±89 &                         1467±111 &                    398±64 &                   232±18 \\
PDDF, basic                &             227±19 &                   278±21 &                   196±28 &                        1199±89 &                           800±29 &                    269±53 &                    166±9 \\
PDDF, fine                 &              192±8 &                   209±15 &                   159±23 &                        1151±68 &                           709±36 &                    287±60 &                   151±19 \\
PDDF, fine+AE              &              190±9 &                   216±12 &                   153±22 &                        1125±66 &                           729±37 &                    267±62 &                    150±8 \\
P²DDF, basic               &             210±16 &                   248±22 &                   200±34 &                        1154±89 &                           786±32 &                   356±110 &                    159±7 \\
P²DDF, fine                &             175±18 &                   184±13 &                    144±9 &                        1084±51 &                           664±45 &                    307±94 &                   142±14 \\
P²DDF, fine+AE             &             171±11 &                   183±15 &                   144±11 &                        1044±52 &                           642±44 &                   308±109 &                    146±9 \\
MBTR, k2-inv               &             171±12 &                   239±32 &                   159±15 &                         917±66 &                           461±43 &                    226±56 &                   150±14 \\
MBTR, k2-rdf               &             173±11 &                   233±38 &                   167±15 &                        1032±62 &                           512±38 &                    197±52 &                   154±12 \\
MBTR, k2-inv-100           &             171±12 &                   240±34 &                   159±16 &                         913±64 &                           466±47 &                    217±45 &                   150±11 \\
MBTR, k2-rdf-100           &             173±15 &                   234±36 &                   164±16 &                        1030±62 &                           506±33 &                    235±69 &                   158±13 \\
MBTR, k2-inv-broad         &             232±25 &                   404±13 &                   170±16 &                        1135±64 &                           586±36 &                    236±65 &                   200±20 \\
MBTR, k2-rdf-broad         &             214±16 &                   350±30 &                   176±18 &                        1152±64 &                           566±31 &                    229±58 &                   182±15 \\
MBTR, full                 &             170±12 &                   238±33 &                   159±15 &                         917±69 &                           461±44 &                    223±59 &                   147±12 \\
MBTR, k2-inv+varsel        &             177±12 &                   265±28 &                   171±19 &                       1064±214 &                           584±69 &                    247±80 &                    145±8 \\
MBTR, k2-rdf+varsel        &             200±14 &                   248±17 &                   208±19 &                       1146±229 &                           641±76 &                    221±65 &                   155±10 \\
MBTR, k2-inv-broad+varsel  &             247±30 &                   410±27 &                   171±13 &                       1413±185 &                          697±121 &                    210±89 &                   211±33 \\
MBTR, k2-rdf-broad+varsel  &             216±19 &                   379±27 &                   188±22 &                        1249±83 &                           663±89 &                    196±71 &                   189±17 \\
MBTR, k2-inv-100+varsel    &             177±11 &                   258±17 &                   166±21 &                       1016±110 &                           583±71 &                    313±70 &                   154±35 \\
MBTR, k2-rdf-100+varsel    &             206±14 &                   261±14 &                   206±16 &                        1072±76 &                           627±61 &                   260±108 &                    156±9 \\
MBTR, full+varsel          &             168±23 &                   231±28 &                  219±101 &                        1018±79 &                           561±56 &                    301±92 &                   143±10 \\
SOAP, Marchenko            &             151±14 &                   158±20 &                   150±11 &                       1713±230 &                           744±78 &                  1431±724 &                   121±13 \\
SOAP, De                   &             148±10 &                   177±24 &                   143±17 &                       1676±222 &                           639±59 &                  1265±637 &                   129±10 \\
SOAP, Nomad                &             149±12 &                   168±28 &                   140±15 &                       1333±136 &                           553±26 &                  1066±727 &                   121±11 \\
SOAP, Nomad, fine          &             247±14 &                   385±10 &                   251±20 &                        1070±76 &                           631±35 &                    216±43 &                   230±16 \\
SOAP, Marchenko, LR        &             181±20 &                   194±27 &                   165±13 &                       2229±393 &                         1805±208 &                 2929±1978 &                    130±9 \\
SOAP, Marchenko+varsel     &             146±11 &                   206±33 &                   161±11 &                         946±58 &                           528±51 &                    252±89 &                   132±32 \\
SOAP, De+varsel            &             158±13 &                   203±16 &                   152±11 &                        1001±62 &                           558±52 &                    253±81 &                   130±12 \\
SOAP, Nomad+varsel         &             151±10 &                   203±38 &                   145±11 &                         944±57 &                           540±48 &                    247±89 &                   130±10 \\
SOAP, Nomad, fine+varsel   &             152±13 &                   207±32 &                   143±12 &                         944±66 &                           521±42 &                   303±147 &                   135±17 \\
SOAP, Marchenko, LR+varsel &             146±13 &                   174±18 &                   138±13 &                         948±60 &                           577±83 &                    253±98 &                   130±10 \\
\bottomrule
\end{tabular}


==> gap_simple_pddfs.tex <==
\begin{tabular}{llll}
\toprule
{} & MAE [meV] & RMSE [meV] &          R² \\
\midrule
  cov\_r\_prod                             &    485±13 &     638±16 &  -0.02±0.11 \\
  ion\_1\_prod                             &    477±28 &     631±32 &   0.23±0.15 \\
  ion\_2\_prod                             &    528±22 &     682±30 &  -0.12±0.17 \\
  r\_prod                                 &    555±19 &     716±22 &  -0.44±0.14 \\
  val\_p\_prod                             &    388±12 &     515±19 &   0.57±0.02 \\
  val\_s\_prod                             &    578±24 &     731±27 &  -0.80±0.25 \\
  vdw\_r\_prod                             &    582±22 &     746±23 &  -0.71±0.16 \\
  e\_prod                                 &    522±22 &     656±30 &   0.03±0.13 \\
  ea\_prod                                &    386±21 &     528±31 &   0.54±0.06 \\
  en\_prod                                &    413±27 &     566±40 &   0.48±0.07 \\
  en+ea\_prod                             &    228±15 &     324±22 &   0.86±0.02 \\
  e+r\_prod                               &    471±18 &     601±11 &   0.28±0.08 \\
  val\_p+val\_s\_prod                       &    419±16 &     526±13 &   0.51±0.06 \\
  ion\_2+ion\_1\_prod                       &    429±19 &     552±23 &   0.43±0.12 \\
  ion\_2+ion\_1+en+ea\_prod                 &     154±9 &     232±20 &   0.93±0.01 \\
  en+ea+e+val\_p+val\_s\_prod               &    138±13 &     220±16 &   0.94±0.01 \\
  ion\_2+ion\_1+en+ea+val\_p+val\_s\_prod     &     126±9 &     188±11 &   0.95±0.01 \\
  ion\_2+ion\_1+en+ea+val\_p+val\_s+e+r\_prod &     116±9 &     184±13 &   0.96±0.01 \\
\bottomrule
\end{tabular}

